RAD-Bench: Evaluating Large Language Models Capabilities in Retrieval Augmented Dialogues

In real-world applications with Large Language Models (LLMs), external retrieval mechanisms - such as Search-Augmented Generation (SAG), tool utilization, and Retrieval-Augmented Generation (RAG) - are often employed to enhance the quality of augmented generations in dialogues. These approaches often come with multi-turn dialogue, where each interaction is enriched by relevant information retrieved from external sources. Existing benchmarks either assess LLMs' chat abilities in multi-turn dialogues or their use of retrieval for augmented responses in single-turn settings. However, there is a gap in evaluating LLMs' ability to leverage retrieval for more precise responses across multiple turns. To address this limitation, we introduce RAD-Bench (Retrieval Augmented Dialogue), a benchmark designed to evaluate LLMs' capabilities in multi-turn dialogues following retrievals, essential for their deployment in context-rich applications. RAD-Bench evaluates two key abilities of LLMs: Retrieval Synthesis and Retrieval Reasoning. These are measured using discriminative questions and retrieved contexts, and corresponding reference answers, assessing how effectively LLMs integrate and reason with context to maintain and enhance conversation quality over multiple turns. Our evaluation results on commonly used LLMs reveal that model performance deteriorates as additional layers of conditions or constraints are applied across conversation turns, even when accurate retrieved contexts are provided. The data and code are available at https://github.com/mtkresearch/RAD-Bench

==> example_samples/customer_support_v0.1.tex <==

    \begin{tabular}{ p{15cm} }
        \toprule
        \textbf{Question 1:} My cash register is displaying an error message 'E' on the screen. What should I do? \\
        \textbf {Context 1:} X - "Read" mode for financial and Cash In Drawer
        
        Z - "Reset" mode for financial and Cash In Drawer
        ...

        C : Indicates the amount displayed is due in change to the customer.
        ...

        If the item to be void is the last item  
        entered, simply press the "VD" key, and the register will remove the very last item entered. When an error occurs, the 'C' key. Error conditions may be caused by incorrect entries or keys pressed in the wrong order. \\
        \midrule
        \textbf{Assistant:} When your cash register displays an error message 'E' on the screen, it indicates an error condition. To clear the error message, you should press the 'C' key. This will help reset the error and allow you to continue operating the cash register. If the error persists, you may want to consult the manual provided for troubleshooting or contact support for further assistance. \\
        \midrule
        \textbf{Question 2:} I pressed the 'C' key, but the error message is still showing. Is it because I pressed the incorrect entries or wrong order? \\
        \textbf{Context 2:} X - "Read" mode for financial and Cash In Drawer
        
        Z - "Reset" mode for financial and Cash In Drawer
        ...

        C : Indicates the amount displayed is due in change to the customer.
        ...

        If the item to be void is the last item  
        entered, simply press the "VD" key, and the register will remove the very last item entered. When an error occurs, the 'C' key. Error conditions may be caused by incorrect entries or keys pressed in the wrong order.  \\
        \midrule
        \textbf{Assistant:} Yes, it's possible that the error message is still showing because you might have pressed the keys in the wrong order or made an incorrect entry. To resolve this, please refer to the manual provided and carefully follow the steps and instructions for the specific error message. Make sure you enter the correct information and follow the order of operations mentioned in the manual. If the error persists, consult the manual for further troubleshooting or contact support for additional assistance. \\
        \midrule
        \textbf{Question 3:} I checked the entries and key order, but the error message 'E' still appears. Could it be a problem with the memory? \\
        \textbf{Context 3:} X - "Read" mode for financial and Cash In Drawer
        
        Z - "Reset" mode for financial and Cash In Drawer
        ...

        C : Indicates the amount displayed is due in change to the customer.
        ...

        If the item to be void is the last item  
        entered, simply press the "VD" key, and the register will remove the very last item entered. When an error occurs, the 'C' key. Error conditions may be caused by incorrect entries or keys pressed in the wrong order. \\
        \midrule  
        \textbf{Assistant:} It's possible that the error message 'E' persists due to a problem with the memory. However, before concluding that it's a memory issue, I recommend you follow the provided context on how to clear the Random Access Memory (RAM) and initialize the cash register. Here are the steps:

        1. Before plugging the register in, place the mode switch in the 'P' position.
        2. Connect the AC plug into a power outlet while pressing the 'C' and '00' keys.
        3. The register should now print a line of decimals ('........').

        This process will clear the RAM of all memory and should be performed only after the battery is first installed. Do not clear the RAM once the register totals will be lost.

        If the error message 'E' still persists after performing this process, consult the manual for further troubleshooting or contact support for additional assistance.\\
        \midrule
    \end{tabular}
